How do annotations affect Java code readability?

Context: Code annotations have gained widespread popularity in programming languages, offering developers the ability to attach metadata to code elements to define custom behaviors. Many modern frameworks and APIs use annotations to keep integration less verbose and located nearer to the corresponding code element. Despite these advantages, practitioners' anecdotal evidence suggests that annotations might negatively affect code readability. Objective: To better understand this effect, this paper systematically investigates the relationship between code annotations and code readability. Method: In a survey with software developers (n=332), we present 15 pairs of Java code snippets with and without code annotations. These pairs were designed considering five categories of annotation used in real-world Java frameworks and APIs. Survey participants selected the code snippet they considered more readable for each pair and answered an open question about how annotations affect the code's readability. Results: Preferences were scattered for all categories of annotation usage, revealing no consensus among participants. The answers were spread even when segregated by participants' programming or annotation-related experience. Nevertheless, some participants showed a consistent preference in favor or against annotations across all categories, which may indicate a personal preference. Our qualitative analysis of the open-ended questions revealed that participants often praise annotation impacts on design, maintainability, and productivity but expressed contrasting views on understandability and code clarity. Conclusions: Software developers and API designers can consider our results when deciding whether to use annotations, equipped with the insight that developers express contrasting views of the annotations' impact on code readability.

==> sections/old-02-backgound.tex <==
\section{Background}
\label{sec:background}

This section briefly describes the leading software engineering concepts necessary for this work, such as program comprehension, code readability, metadata, and annotation. 

\textbf{Program Comprehension} is an essential aspect of software maintenance and supports software evolution~\citep{STOREY2000183}. Comprehending the source code and the structure of a system is required before applying any proper modification or enhancement~\citep{7961527}. Developers can use different artifacts to help to comprehend a program, including the source code~\citep{STOREY2000183}, which should offer high readability.

\textbf{Readability} can be defined as \textit{``a human judgment of how easy a text is to understand''}~\citep{Buse2010}. Code readability is an essential component of program comprehension~\citep{lucas2019does, Rugaber00} and is directly related to its maintainability~\citep{Buse2010}. Development teams pursue this quality attribute since the typical software product life-cycle cost distribution is 70\% maintenance and 30\% development~\citep{Boehm2001}. Moreover, other studies indicate that source code reading is the most time-consuming process of all maintenance activities~\citep{Raymond1991, Rugaber00}. Metadata can enhance the readability of the source code.

The term \textbf{``metadata''} is used in various contexts in computer science, meaning data about the data itself. In the object-oriented context, metadata includes the information that describes the class. Some tools or frameworks can consume metadata and execute routines based on class structure. For instance, it can be used for source code generation~\citep{Damyanov2004}, compile-time verification~\citep{Ernst2008,Quinonez2008}, class transformation \footnote{\url{http://projectlombok.org}}, and framework adaptation~\citep{Guerra2010b}. 

The metadata can be defined through the usage of object-oriented techniques. The presence of an interface can define a class property. It is a practice called marking interface~\citep{bloch2016effective}. Class metadata can also be returned as fixed information from static methods or set in static variables with name conventions. Alternatively, an object containing the metadata might be created programmatically by setting the appropriate information~\citep{guerra2013reference}. Finally, as another option, metadata can be passed using fixed literals as arguments to methods that rely on them, usually executed as an initialization code.

An approach to defining custom metadata is to use external resources, such as configuration files or databases~\citep{Fernandes2010}. The drawback of this approach is the distance between the metadata and the referred code element. That also adds some verbosity since a complete path to the element must be provided so that the framework may correctly consume the metadata. Some frameworks, like Ruby on Rails and the CakePHP, use an alternative to define behavior through code conventions~\citep{Chen}. Although this choice can be productive in some contexts, code conventions have limited expressiveness. Moreover, since the metadata is hidden behind the conventions, an unwary developer might alter it, causing unwanted effects.

Some programming languages provide features that allow custom metadata to be defined and included directly on programming elements. This feature is supported in languages such as Java, through annotations, and in C\#, by attributes. Since metadata definition is closer to the programming element, it is less verbose than an external definition. 

\textbf{Annotations} were introduced as a language feature in Java 1.5. Some standard APIs like EJB (Enterprise Java Beans) 3.0, JPA (Java Persistence API), and CDI (Context and Dependency Injection) extensively use metadata in the form of annotations. This native annotation support encouraged Java frameworks and API developers to adopt the metadata-based approach in their solutions. That confirmed the tendency to keep the metadata files inside the source code instead of using separate files~\citep{CORDOBASANCHEZ2016}.

An annotation-based API, or metadata-based framework, define and expose a set of annotations so application developers can use them to configure programming elements and execute the desired behavior. This set of annotations that define a metadata structure of a given domain for an API is defined as \textbf{annotation schema}~\citep{lima2018jss}. For instance, the annotation schema for object-relational mapping of the JPA API includes the annotations like \texttt{@Table}, \texttt{@Column}, \texttt{@Id}, and \texttt{@OneToMany}.

The code annotations from the same schema are usually located in the same Java package. In the example of the JPA API, all the object-relational mapping annotations are located on \texttt{javax.persistence}. Based on that, \cite{lima2018jss} suggests the heuristic of using the package to identify and name the annotation schema. Accordingly, we would say that \texttt{@Table} and \texttt{@Column} belong to the annotation schema \texttt{javax.persistence}. Moreover, the same API or framework might define multiple packages with annotations representing metadata with different purposes. In this case, each package represents a different annotation schema. For instance, the \texttt{javax.persistence.metamodel} is an example of another annotation schema that belongs to the JPA API. In this paper, we adopted the same heuristic from \cite{lima2018jss} and used the annotation package to identify its annotation schema. 

==> sections/old-03-related-work.tex <==
\section{Related Work}
\label{sec:related_work}

Although no previous work discusses the impacts of code annotation on code readability, there are \textbf{studies discussing code readability in multiple ways}. Moreover, although we did not find other works that investigated the impact of annotations on code readability, there are \textbf{studies that investigated other quality attributes that can influence or be influenced by it}. This section presents and discusses these studies as closer to our investigation.

\subsection{Code Readability}

In the following, we discuss two studies that investigated code readability through surveys in which participants compared the readability of pairs of code snippets.

\cite{dos2018impacts} conducted a survey that assessed the impact of Java coding practices and conventions on the readability perceived by software developers. They did not investigate code annotations. Their results helped to identify practices and conventions with positive and negative impacts on readability and, thus, can guide the definition of coding standards. 

\cite{lucas2019does} present a mixed-method study using quantitative and qualitative methods to evaluate the effects on Java code comprehension in methods before and after using lambda expressions. Their quantitative analysis was based on two models for estimating code readability \citep{Buse2010, Posnett2011} by evaluating source code complexity and readability metrics. Their study was based on an online survey where participants evaluated pairs of code snippets. 
The survey indicated that introducing lambda expressions on legacy code improved its readability. 

\subsection{Annotated Code Assessment}

In the context of quality attributes that can influence or be influenced by the annotations,~\cite{guerra2013qualitative} assessed the impact of frameworks based on annotations compared to object-oriented frameworks. Similar to the present work, it considered patterns for annotation usage to design the scenarios. The study did not conclude that annotations lead to reduced coupling and that the indirection of metadata definition leads to difficulty debugging.  

\cite{lima2018jss} proposed a suite of software metrics to characterize code annotations' complexity, coupling, and size. Based on data from 25 open-source Java projects, they observed that 78\% of classes contain at least one annotation, highlighting the relevance of studying the impact of their presence. Identifying metric outliers, such as a class with 729 code annotations and one annotation that took 58 lines of code, reveals abuses in using this language feature. 

\cite{Yu2019} performed a large-scale empirical study on code annotations usage, evolution, and impact. The authors collected data from 1094 open-source Java projects and conducted a historical analysis to assess code annotations. One of the findings revealed a high number of changes in annotations during project evolution, implicating that some developers tend to use annotations subjectively and arbitrarily, introducing code problems. The study also revealed that developers intending to improve code readability add annotations to the existing program elements. By relating annotation usage to code error-proneness, the study concluded that they could potentially enhance software quality by relating annotation usage to code error-proneness.

Concerning annotation repetition,~\cite{teixeira2018does} performed a study investigating the source code of a set of web applications searching for annotations being repeated throughout the source code. The findings revealed that some annotations were repeated around 100 times in code elements with shared characteristics in the target system. The study suggested that more general definitions, such as application-specific code conventions, could significantly reduce the number of configurations.

A recent experiment about framework development compared the usage of an annotation-based API to another based on object orientation for metadata reading~\citep{guerra2020}. The results showed a more consistent behavior in the evolution of coupling and complexity metrics when using the annotation-based approach, but they did not find significant differences in productivity. 

The work of~\cite{Lima2022cadv} proposed a software visualization approach to observe how code annotations are distributed in a given system and improve code comprehension of annotation-based systems. The authors conducted an empirical evaluation with students and professional developers using a Java web application as the target system. From their findings, the authors observed a strong relationship between the presence of a code annotation and the responsibility of the package/class using that annotation. This finding suggests that code annotations may also guide the architectural design of software systems.

In conclusion, based on the studies found in the literature, from the positive side, the usage of annotations can reduce coupling~\citep{guerra2013qualitative}, provide a more consistent evolution~\citep{guerra2020}, and potentially improve code quality~\citep{Yu2019}. On the other hand, the studies showed abuses in their application related to size~\citep{lima2018jss} and repetition~\citep{teixeira2018does}. Moreover, annotations can make debugging harder~\citep{guerra2013qualitative} and introduce code problems when introduced arbitrarily by developers~\citep{Yu2019}. However, no prior study focused on developers' perceptions regarding the readability of code with and without annotations, which is the goal of this study.
